GenAssist: Making Image Generation Accessible

Blind and low vision (BLV) creators use images to communicate with sighted audiences. However, creating or retrieving images is challenging for BLV creators as it is difficult to use authoring tools or assess image search results. Thus, creators limit the types of images they create or recruit sighted collaborators. While text-to-image generation models let creators generate high-fidelity images based on a text description (i.e. prompt), it is difficult to assess the content and quality of generated images. We present GenAssist, a system to make text-to-image generation accessible. Using our interface, creators can verify whether generated image candidates followed the prompt, access additional details in the image not specified in the prompt, and skim a summary of similarities and differences between image candidates. To power the interface, GenAssist uses a large language model to generate visual questions, vision-language models to extract answers, and a large language model to summarize the results. Our study with 12 BLV creators demonstrated that GenAssist enables and simplifies the process of image selection and generation, making visual authoring more accessible to all.

==> sections/extra-stuff.tex <==
Introduction

% To better understand the opportunities and the requirements of the accessible Text-to-Image generation system, we conducted a formative study with eight people with visual impairments who regularly create or search for images. In the\amy{``our'' or ``a''... ``the'' makes it sound like we're referring to something we've mentioned before, or it was already existing} two-stage formative study, we first interviewed participants about their current video creation/search strategies and challenges, then the participants experienced generating\amy{``experienced generationg'' --> ``generated''} images using a Text-to-Image generation model. 

System

we present two tables: \textbf{visual content table} where the information of setting, subjects, emotion, potential image use case, and detected objects is provided, and the \textbf{visual attributes table} where the information about the medium, lighting, perspective, colors, and errors is provided. Our choice of the type of information covered in these two tables is based on an analysis of existing TTI guidelines\footnote{https://docs.midjourney.com/docs/prompts}\footnote{https://github.com/willwulfken/MidJourney-Styles-and-Keywords-Reference}\footnote{https://dallery.gallery/the-dalle-2-prompt-book/}. In addition, we also included ``detected objects'' as it was often asked by the formative study participants who were using TTI model. Also, ``error'' information was added to surface any distortion in the generated images such as blurring or unnatural human body features. 

% Prompts that specify the content and style of the desired image help to text-to-image generation models produce images that closely follow the prompt\footnote{https://docs.midjourney.com/docs/prompts}\footnote{https://github.com/willwulfken/MidJourney-Styles-and-Keywords-Reference}\footnote{https://dallery.gallery/the-dalle-2-prompt-book/}. When prompts are short or leave aspects of the image underspecified, the text-to-image model fills in the remaining details. For example, Vito's prompt \textit{``A young chef is cooking dinner for his parents''} does not specify the style such that the resulting images include three illustrations and one photo. As a result, many of the similarities and differences between the image candidates are not captured by prompt verification alone.
% Text-to-image prompt guidelines\footnote{https://docs.midjourney.com/docs/prompts}\footnote{https://github.com/willwulfken/MidJourney-Styles-and-Keywords-Reference}\footnote{https://dallery.gallery/the-dalle-2-prompt-book/} request that users specify the content and style of their desired images to help text-to-image models follow the prompts.
% However, when users provide short, underspecified prompts, text-to-images models produce images by filling in the remaining details. As a result, many of the similarities and differences between the image candidates are not captured by prompt verification alone. For example, Vito's image candidates for his prompt \textit{``A young chef is cooking dinner for his parents''} portreyed varying styles including three illustrations and one photo.
 % A well-crafted prompt that follows existing prompt guidelinescan help text-to-image models produce images that closely reflect the specified content and style of the prompt. However, when users input short prompts that do not fully specify the desired content and style of the image, the model fills in remaining details such that the resulting images have many differences that are not captured by prompt verification alone.


 
% The participants described their vision as either totally blind (10 participants) or legally blind (2 participants) and they represented varied professions encompassing students, consultants, software engineers, video creators, and artists. Two of the participants also participated in the formative study (P7, P8). 
% Our 1.5-hour remote Zoom study using mailing lists. using mailing lists. Participants were compensated 50 USD for the 1.5-hour remote study conducted via Zoom\footnote{https://zoom.us/}. We audio recorded and transcribed the study, and the study was approved by our institution's IRB. 

% \subsection{Procedure}


% \subsubsection{Materials}
% In the interpretation task, participants used one of the two interface conditions to understand a set of pre-generated images. From the Midjourney's community feed, we selected two sets of images generated with a short prompt (S1, S3 in \autoref{fig:materials}- without detailed descriptions of objects or styles) and two sets with a long prompt (S2, S4 in \autoref{fig:materials}- detailed descriptions of objects or styles). We included both short prompt images and long prompt images to test our system with input images that are diverse as well as those that are similar to each other \amy{might not be clear which is which -- long prompt creates images that are closer together probably?}. 

% In the generation task, participants read two news articles and came up with their own prompt to create images relevant to the articles. We selected two articles from the New York Times: 1) Why Multitasking is Bad for You~\footnote{https://time.com/4737286/multitasking-mental-health-stress-texting-depression/} and 2) My Kids Want Plastic Toys. I Want to Go Green. Here's the Middle Ground~\footnote{https://time.com/6126981/my-kids-want-plastic-toys-i-want-to-go-green-heres-a-fix/}. The first article had an illustration image while the second article featured a photo to convey the idea. From both articles, we extracted the title and five paragraphs to constitute a rough summary of the original article. 

% \subsubsection{Procedure}
% % We conducted a 90-minute remote study on Zoom\footnote{https://zoom.us/} where all participants had a 1:1 session with one of the researchers. 
% We first asked participants demographic and background questions about how they use images in their work. We then gave a 15-minute tutorial on both the \sysname{} interface and the baseline interface.
% The baseline interface provided for each image: the image caption (generated with BLIP-2), a list of objects in the image (detected with Detic), and the ability to ask visual questions about the image (answered by BLIP-2). 
% % The baseline interface did not have the four tables (summary caption, prompt-verification, visual content, visual attributes) of the \sysname. 
% % Instead, the baseline interface provided the default image caption (generated with BLIP-2) as well as the list of objects in the image (detected with Detic). 
% % Users could also ask additional visual questions about individual images which were answered by the BLIP-2 model. 

% \ipstart{Interpretation Task}
% In the interpretation task, participants experienced both interface conditions to understand and evaluate pre-generated images. For each set of images, we provided participants with an example scenario of using the image (\textit{e.g.,} a blog post titled ``My grandma still dances!'' for S2). After reading the description provided by \sysname{} or the baseline interface, participants were asked to summarize the differences and choose one final image. For each interface, users were given one shot prompt images (S1 or S3) and one long prompt images (S2 or S4). The orders of interface type (\sysname{} and baseline) and image type were counterbalanced and randomly assigned to participants. After each interface, we conducted a post-stimulus survey that included the following ratings: Mental Demand, Performance, Effort, Frustration, and Usefulness of the caption in understanding differences between images. All ratings were on a 7-point Likert scale.


% \ipstart{Generation Task}
%  In the following generation task, participants were given two articles and created relevant images by coming up with their own prompts. The orders of interface type (\sysname{} and baseline) and article type were counterbalanced and randomly assigned to participants. After each interface, we asked the participants to choose one image from the generated images and explain the reason. We also conducted a post-stimulus survey that included the following ratings: Mental Demand, Performance, Effort, Frustration, Usefulness of the caption, Satisfaction with the final image, and Confidence in posting the final image. All ratings were on a 7-point Likert scale. At the end of the study, we conducted a semi-structured interview to understand participants' strategies using ~\sysname{} and the pros and cons of both ~\sysname{} and the baseline.

% \subsubsection{Analysis}
% We collected the video recordings, the interaction logs, user-generated prompts and images, and the survey responses to perform both quantitative and qualitative analyses. 
% \sysname{}'s interaction logs were collected using Google Firebase~\cite{firebase}. We transcribed the exit interviews and participants' spontaneous comments during the tasks and grouped the transcript according to (1) strategies of using \sysname{} and (2) perceived benefits and limitations of our system.


